A Generalized Modality for Recursion

Nakano's later modality allows types to express that the output of a function does not immediately depend on its input, and thus that computing its fixpoint is safe. This idea, guarded recursion, has proved useful in various contexts, from functional programming with infinite data structures to formulations of step-indexing internal to type theory. Categorical models have revealed that the later modality corresponds in essence to a simple reindexing of the discrete time scale. Unfortunately, existing guarded type theories suffer from significant limitations for programming purposes. These limitations stem from the fact that the later modality is not expressive enough to capture precise input-output dependencies of functions. As a consequence, guarded type theories reject many productive definitions. Combining insights from guarded type theories and synchronous programming languages, we propose a new modality for guarded recursion. This modality can apply any well-behaved reindexing of the time scale to a type. We call such reindexings time warps. Several modalities from the literature, including later, correspond to fixed time warps, and thus arise as special cases of ours.

==> fig-alg-division.tex <==
\begin{figure}
  \begin{mathpar}
    \fbox{\algD{\tau}{p}{\tau'}{\alpha}}

    \IRULE
    {
      ~
    }
    {
      \algD
      {\tyW{q}{\tau}}
      {p}
      {\tyW{q \wD p}{\tau}}
      {\coeDEL{q}{p \opON (q \wD p)};\coeDECAT{p}{q \,\wD p}}
    }

    \IRULE
    {
      \algD
      {\tau_1}
      {p}
      {\tau_1'}
      {\alpha_1}
      \\
      \algD
      {\tau_2}
      {p}
      {\tau_2'}
      {\alpha_2}
    }
    {
      \algD
      {\tyPROD{\tau_1}{\tau_2}}
      {p}
      {\tyPROD{\tau_1'}{\tau_2'}}
      {\coePROD{\alpha_1}{\alpha_2}}
    }

    \fbox{\algD{\Gamma}{p}{\Gamma'}{\gamma}}

    \IRULE
    {
      ~
    }
    {
      \algD
      {\ctxempty}
      {p}
      {\ctxempty}
      {\emptyset}
    }

    \IRULE
    {
      \algD
      {\Gamma}
      {p}
      {\Gamma'}
      {\gamma}
      \\
      \algD
      {\NORMty{\tau}}
      {p}
      {\tau'}
      {\alpha}
    }
    {
      \algD
      {\Gamma, x : \tau}
      {p}
      {\Gamma', x : \tau'}
      {\gamma[x \mapsto \NORMin{\tau};\alpha]}
    }
  \end{mathpar}
%  \small
  % \begin{center}
  %   \fbox{$\tau \wD p$} and \fbox{$\Gamma \wD p$}
  % \end{center}
  % \begin{align*}
  %   (\tyW{q}{\tau}) \wD p
  %   & =
  %   (\tyW{q \wD p}{\tau},
  %   (\coeDEL{q}{p \opON\, (q \wD p)};
  %   \coeDECAT{p}{q \wD p}))
  %   \\
  %   (\tyPROD{\tau_1}{\tau_2}) \wD p
  %   & =
  %   (\tyPROD{\tau_1'}{\tau_2'}, \coePROD{\alpha_1}{\alpha_2})
  %   \mbox{ where }
  %   \begin{array}[t]{@{}l}
  %     (\tau_1,\alpha_1) = \tau_1 \wD p
  %     \\
  %     (\tau_2,\alpha_2) = \tau_2 \wD p
  %   \end{array}
  %   \\
  %   \ctxempty \wD p
  %   & = (\ctxempty, \emptyset)
  %   \\
  %   (\Gamma, x : \tau) \wD p
  %   & =
  %   ((\Gamma', x : \tau'), \gamma[x \mapsto \NORMin{\tau};\alpha])
  %   \mbox{ where }
  %   \begin{array}[t]{@{}l}
  %     (\Gamma',\gamma) = \Gamma \wD p
  %     \\
  %     (\tau', \alpha) = \NORMty{\tau} \wD p
  %   \end{array}
  % \end{align*}
  \caption{Type and Context Division}
  \label{fig:alg-division}
\end{figure}


==> fig-alg-precedence.tex <==
\begin{figure}
  \[
    \begin{array}{r@{\;}c@{\;}l}
      % \Coe{\tau_1}{\tau_2}
      % & = &
      % \NORMin{\tau_1}
      % ;
      % \Prec{\NORM{\tau_1}}{\NORM{\tau_2}}
      % ;
      % \NORMout{\tau_2}
      % \\
      \Prec{\nu}{\nu}
      & = &
      \coeID
      \\
      \Prec
      {\tyS{\tau_1}}
      {\tyS{\tau_2}}
      & = &
      \coeS{\Prec{\tau_1}{\tau_2}}
      \\
      \Prec
      {\tyARR{\tau_1'}{\tau_1''}}
      {\tyARR{\tau_2'}{\tau_2''}}
      & = &
      \coeARR
      {\Prec{\tau_2'}{\tau_1'}}
      {\Prec{\tau_1''}{\tau_2''}}
      \\
      \Prec
      {\tyPROD{\tau_1'}{\tau_1''}}
      {\tyPROD{\tau_2'}{\tau_2''}}
      & = &
      \coePROD
      {\Prec{\tau_1'}{\tau_2'}}
      {\Prec{\tau_1''}{\tau_2''}}
      \\
      \Prec
      {\tySUM{\tau_1'}{\tau_1''}}
      {\tySUM{\tau_2'}{\tau_2''}}
      & = &
      \coeSUM
      {\Prec{\tau_1'}{\tau_2'}}
      {\Prec{\tau_1''}{\tau_2''}}
      \\
      \Prec
      {\tyW{p}{\tau_1}}
      {\tyW{q}{\tau_2}}
      & = &
      \coeDEL{p}{q}
      ;
      \coeW{q}{\Prec{\tau_1}{\tau_2}}
      \mbox{ if } p \ge q
    \end{array}
  \]
  \caption{Type Precedence}
  \label{fig:alg-precedence}
\end{figure}


==> fig-alg-simplification.tex <==
\begin{figure}
  \begin{align*}
    \NORM{\nu}
    & = \tyW{\wOM}{\nu}
    \\
    \NORM{\tyS{\tau}}
    & =
    \tyW{\wID}{\tyS{\NORM{\tau}}}
    \\
    \NORM{\tyARR{\tau_1}{\tau_2}}
    & =
    \tyW{\wID}{(\tyARR{\NORM{\tau_1}}{\NORM{\tau_2}})}
    \\
    \NORM{\tyPROD{\tau_1}{\tau_2}}
    & =
    \tyPROD{\NORM{\tau_1}}{\NORM{\tau_2}}
    \\
    \NORM{\tySUM{\tau_1}{\tau_2}}
    & =
    \tyW{\wID}{(\tySUM{\NORM{\tau_1}}{\NORM{\tau_2}})}
    \\
    \NORM{\tyW{p}{\tyW{q}{\tau}}}
    & =
    \NORM{\tyW{p \opON q}{\tau}}
    \\
    \NORM{\tyW{p}{(\tyPROD{\tau_1}{\tau_2})}}
    & =
    \tyPROD{\NORM{\tyW{p}{\tau_1}}}{\NORM{\tyW{p}{\tau_2}}}
    \\
    \NORM{\tyW{p}{\tau}}
    & =
    \tyW{p \opON q}{\tau'}
    \mbox{ where }
    \tyW{q}{\tau'} = \NORM{\tau}
    % \\
    % \NORM{\tyW{p}{\tau}}
    % & =
    % \left\{
    %   \begin{array}{@{}l@{~}l}
    %     \tyPROD{\NORM{\tyW{p}{\tau_1}}}{\NORM{\tyW{p}{\tau_2}}}
    %     &
    %     \mbox{if } \tyPROD{\tau_1}{\tau_2} = \NORM{\tau}
    %     \\
    %     \tyW{p \opON q}{\tau'}
    %     &
    %     \mbox{if } \tyW{q}{\tau'} = \NORM{\tau}
    %   \end{array}
    % \right.
  \end{align*}
  % \begin{align*}
  %   \NORM{\nu}
  %   & = (\tyW{\wOM}{\nu}, \coeINFL, (\coeDEL{\wOM}{\wID};\coeUNWRAP))
  %   \\
  %   \NORM{\tyS{\tau}}
  %   & =
  %   \begin{array}[t]{@{}l}
  %     (\tyW{\wID}{\tyS{\tau'}},
  %     (\coeS{\alpha};\coeWRAP),
  %     (\coeUNWRAP;\coeS{\alpha'}))
  %     \\
  %     \mbox{where }
  %     (\tau',\alpha,\alpha') = \NORM{\tau}
  %   \end{array}
  %   \\
  %   \NORM{\tyARR{\tau_1}{\tau_2}}
  %   & =
  %   \begin{array}[t]{@{}l}
  %     (\tyW{\wID}{(\tyARR{\tau_1'}{\tau_2'})},
  %     (\coeARR{\alpha_1'}{\alpha_2};\coeWRAP),
  %     (\coeUNWRAP;\coeARR{\alpha_1}{\alpha_2'}))
  %     \\
  %     \mbox{where }
  %     (\tau_1',\alpha_1,\alpha_1') = \NORM{\tau_1}
  %     \mbox{ and }
  %     (\tau_2',\alpha_2,\alpha_2') = \NORM{\tau_2}
  %   \end{array}
  %   \\
  %   \NORM{\tyPROD{\tau_1}{\tau_2}}
  %   & =
  %   \begin{array}[t]{@{}l}
  %     (\tyPROD{\tau_1'}{\tau_2'},
  %     \coePROD{\alpha_1}{\alpha_2},
  %     \coePROD{\alpha_1'}{\alpha_2'})
  %     \\
  %     \mbox{where }
  %     (\tau_1',\alpha_1,\alpha_1') = \NORM{\tau_1}
  %     \mbox{ and }
  %     (\tau_2',\alpha_2,\alpha_2') = \NORM{\tau_2}
  %   \end{array}
  %   \\
  %   \NORM{\tySUM{\tau_1}{\tau_2}}
  %   & =
  %   \begin{array}[t]{@{}l}
  %     (\tyW{\wID}{(\tySUM{\tau_1'}{\tau_2'})},
  %     (\coeSUM{\alpha_1}{\alpha_2};\coeWRAP),
  %     (\coeUNWRAP;\coeSUM{\alpha_1'}{\alpha_2'}))
  %     \\
  %     \mbox{where }
  %     (\tau_1',\alpha_1,\alpha_1') = \NORM{\tau_1}
  %     \mbox{ and }
  %     (\tau_2',\alpha_2,\alpha_2') = \NORM{\tau_2}
  %   \end{array}
  %   \\
  %   \NORM{\tyW{p}{(\tyPROD{\tau_1}{\tau_2})}}
  %   & =
  %   \begin{array}[t]{@{}l}
  %     (\tau', (\coeDISTP;\alpha), (\alpha';\coeFACTP))
  %     \\
  %     \mbox{where }
  %     (\tau',\alpha,\alpha')
  %     =
  %     \NORM{\tyPROD{\tyW{p}{\tau_1}}{\tyW{p}{\tau_2}}}
  %   \end{array}
  %   \\
  %   \NORM{\tyW{p}{\tau}}
  %   & =
  %   \begin{array}[t]{@{}l}
  %     (\tyW{p \opON q}{\tau'},
  %     (\coeW{p}{\alpha};\coeCONCAT{p}{q}),
  %     (\coeDECAT{p}{q};\coeW{p}{\alpha'}))
  %     \\
  %     \mbox{if }  \tau \ne (\tyPROD{\_}{\_})
  %     \mbox{ and with }
  %     (\tyW{q}{\tau'},\alpha,\alpha')
  %     =
  %     \NORM{\tau}
  %   \end{array}
  % \end{align*}
  \caption{Type Normalization}
  \label{fig:alg-simplification}
\end{figure}


==> fig-alg-type-checking.tex <==
\begin{figure*}
  \begin{mathpar}
    \fbox{$\algT{\Gamma}{t}{\tau}{e}$}

    \IRULE[AlgVar]
    {
      \Gamma(x) = \tau
    }
    {
      \algT
      {\Gamma}
      {x}
      {\tau}
      {x}
    }

    \IRULE[AlgFun]
    {
      \algT
      {\Gamma, x : \tau}
      {t}
      {\tau'}
      {e}
    }
    {
      \algT
      {\Gamma}
      {\synFUN{x}{\tau}{t}}
      {\tyARR{\tau}{\tau'}}
      {\synFUN{x}{\tau}{e}}
    }

    \IRULE[AlgApp]
    {
      \algT
      {\Gamma}
      {t_1}
      {\tau_1}
      {e_1}
      \\
      \algT
      {\Gamma}
      {t_2}
      {\tau_2}
      {e_2}
      \\
      \algIa
      {\tau_1}
      {\tau_1'}
      {\tau_1''}
      {\alpha_1}
      \\
      \algC
      {\tau_2}
      {\tau_1'}
      {\alpha_2}
    }
    {
      \algT
      {\Gamma}
      {t_1~t_2}
      {\tau_2}
      {(e_1;\alpha_1)~(e_2;\alpha_2)}
    }

    \IRULE[AlgPair]
    {
      \algT
      {\Gamma}
      {t_1}
      {\tau_1}
      {e_1}
      \\
      \algT
      {\Gamma}
      {t_2}
      {\tau_2}
      {e_2}
    }
    {
      \algT
      {\Gamma}
      {(t_1, t_2)}
      {\tyPROD{\tau_1}{\tau_2}}
      {(e_1, e_2)}
    }

    \IRULE[AlgProj$_{i \in \{1, 2\}}$]
    {
      \algT
      {\Gamma}
      {t}
      {\tau}
      {e}
      \\
      \algIp
      {\tau}
      {\tau_1}{\tau_2}
      {\alpha}
    }
    {
      \algT
      {\Gamma}
      {\synPROJ{i}{t}}
      {\tau_i}
      {\synPROJ{i}{(e;\alpha)}}
    }

    \IRULE[AlgInj$_{i \in \{0, 1\}}$]
    {
      \algT
      {\Gamma}
      {t}
      {\tau_i}
      {e}
    }
    {
      \algT
      {\Gamma}
      {\synINJ{i+1}{\tau_{1-i}}{t}}
      {\tySUM{\tau_0}{\tau_1}}
      {\synPROJ{i+1}{e}}
    }

    % \IRULE[AlgInj$_2$]
    % {
    %   \algT
    %   {\Gamma}
    %   {t}
    %   {\tau_2}
    %   {e}
    % }
    % {
    %   \algT
    %   {\Gamma}
    %   {\synINJ{1}{\tau_1}{t}}
    %   {\tySUM{\tau_1}{\tau_2}}
    %   {\synPROJ{2}{e}}
    % }

    \IRULE[AlgCase]
    {
      \algT
      {\Gamma}
      {t}
      {\tau}
      {e}
      \\
      \algIs
      {\tau}
      {\tau_1}{\tau_2}
      {\alpha}
      \\
      (\algT
      {\Gamma, x : \tau_i}
      {t_i}
      {\tau_i'}
      {e_i})_{i \in \{1, 2\}}
      \\
      (\tau_i' = \NORMty{\tau_i})_{i \in \{1, 2\}}
      \\
      (\alpha_i = \NORMin{\tau_i})_{i \in \{1, 2\}}
    }
    {
      \algT
      {\Gamma}
      {\synCASE{t}{x_1}{t_1}{x_2}{t_2}}
      {\SUP{\tau_1'}{\tau_2'}}
      {
        \synCASE
        {e;\alpha}
        {x_1}{e_1;\alpha_1;\SUPl{\tau_1'}{\tau_2'}}
        {x_2}{e_2;\alpha_2;\SUPr{\tau_1'}{\tau_2'}}
      }
    }

    \IRULE[AlgScal]
    {
      s \in \SCAL_\nu
    }
    {
      \algT
      {\Gamma}
      {s}
      {\nu}
      {s}
    }

    \IRULE[AlgRec]
    {
      \algT
      {\Gamma, x : \tyW{\wPRED}{\tau}}
      {t}
      {\tau'}
      {e}
      \\
      \algC
      {\tau'}
      {\tau}
      {\alpha}
    }
    {
      \algT
      {\Gamma}
      {\synREC{x}{\tau}{t}}
      {\tau}
      {\synREC{x}{\tau}{(e;\alpha)}}
    }

    \IRULE[AlgWarp]
    {
      \algD
      {\Gamma}
      {p}
      {\Gamma'}
      {\beta}
      \\
      \algT
      {\Gamma'}
      {t}
      {\tau}
      {e}
    }
    {
      \algT
      {\Gamma}
      {\synBY{t}{p}}
      {\tyW{p}{\tau}}
      {
        \beta;(\synBY{e}{p})
      }
    }
  \end{mathpar}
  \caption{Abstract Type-Checking Algorithm}
  \label{fig:alg-type-checking}
\end{figure*}


==> fig-context-subtyping.tex <==
\begin{figure}
  \begin{mathpar}
    \fbox{$\jugC{\beta}{\Gamma}{\Gamma'}$}

    \IRULE
    {
      ~
    }
    {
      \jugC{\beta}{\ctxempty}{\ctxempty}
    }

    \IRULE
    {
      \jugC{\beta}{\Gamma}{\Gamma'}
      \\
      \jugC{\beta(x)}{\tau}{\tau'}
    }
    {
      \jugC{\beta}{\Gamma, x : \tau}{\Gamma', x : \tau'}
    }
  \end{mathpar}
  \caption{Context Subtyping Judgment}
  \label{fig:context-subtyping}
\end{figure}


==> fig-logical-relation.tex <==
\begin{figure}
  \fbox{$\IMPL{\tau}{n} \subseteq \opsem{\tau}(n) \times \sem{\tau}(n)$}
  \begin{align*}
    c \IMPL{\tyG{\nu}}{n} c
    \\
    (\vC{v_1}{v_2}) \IMPL{\tyS{\tau}}{n+1} (x_1,x_2)
    & \Leftrightarrow
    v_1 \IMPL{\tau}{n+1} x
    \wedge
    v_2 \IMPL{\tyS{\tau}}{n} x
  \end{align*}
  \caption{Logical Relation for Adequacy}
  \label{fig:logical-relation}
\end{figure}


==> fig-streams.tex <==
\begin{figure*}
  \begin{mathpar}
    \IRULE[Head]
    {
      \jugT
      {\Gamma}
      {e}
      {\tyS{\tau}}
    }
    {
      \jugT
      {\Gamma}
      {\synHEAD{e}}
      {\tau}
    }

    \IRULE[Tail]
    {
      \jugT
      {\Gamma}
      {e}
      {\tyS{\tau}}
    }
    {
      \jugT
      {\Gamma}
      {\synTAIL{e}}
      {\tyW{\wPRED}{\tyS{\tau}}}
    }

    \IRULE[Cons]
    {
      \jugT
      {\Gamma}
      {e_1}
      {\tau}
      \\
      \jugT
      {\Gamma}
      {e_2}
      {\tyW{\wPRED}{\tyS{\tau_2}}}
    }
    {
      \jugT
      {\Gamma}
      {\synCONS{e_1}{e_2}}
      {\tyS{\tau}}
    }
  \end{mathpar}
  \begin{center}
    (A) - Typing Judgment
  \end{center}
  \begin{mathpar}
    \IRULE[EHead]
    {
      \jugEV
      {e}
      {\gamma}
      {n+1}
      {\vC{v_1}{v_2}}
    }
    {
      \jugEV
      {\synHEAD{e}}
      {\gamma}
      {n+1}
      {v_1}
    }

    \IRULE[ECons]
    {
      \jugEV
      {e}
      {\gamma}
      {n+1}
      {\vC{v_1}{v_2}}
    }
    {
      \jugEV
      {\synTAIL{e}}
      {\gamma}
      {n+1}
      {\vW{\wPRED}{v_2}}
    }

    \IRULE[ECons]
    {
      \jugEV
      {e_1}
      {\gamma}
      {n+1}
      {v_1}
      \\
      \jugEV
      {e_2}
      {\gamma}
      {n+1}
      {\vW{\wPRED}{v_2}}
    }
    {
      \jugEV
      {\synCONS{e_1}{e_2}}
      {\gamma}
      {n+1}
      {\vC{v_1}{v_2}}
    }
  \end{mathpar}
  \begin{center}
    (B) - Evaluation Judgment
  \end{center}
  \begin{mathpar}
    \IRULE[AlgHead]
    {
      \algT
      {\Gamma}
      {t}
      {\tau}
      {e}
      \\
      \algIS
      {\tau}
      {\tau'}
      {\alpha}
    }
    {
      \algT
      {\Gamma}
      {\synHEAD{t}}
      {\tau}
      {\synHEAD{(e;\alpha)}}
    }

    \IRULE[AlgTail]
    {
      \algT
      {\Gamma}
      {t}
      {\tau}
      {e}
      \\
      \algISP
      {\tau}
      {\tau'}
      {\alpha}
    }
    {
      \algT
      {\Gamma}
      {\synTAIL{t}}
      {\tau}
      {\synTAIL{(e;\alpha)}}
    }

    \IRULE[AlgCons]
    {
      \algT
      {\Gamma}
      {t_1}
      {\tau_1}
      {e_1}
      \\
      \algT
      {\Gamma}
      {t_2}
      {\tau_2}
      {e_2}
      \\
      \algISP
      {\tau_2}
      {\tau}
      {\alpha}
    }
    {
      \algT
      {\Gamma}
      {\synCONS{t_1}{t_2}}
      {\SUP{\tau_1}{\tau}}
      {
        \synCONS
        {(t_1;\SUPl{\tau_1}{\tau})}
        {(t_2;\alpha;\coeW{\wPRED}{\coeS{(\SUPr{\tau_1}{\tau})}})}
      }
    }
  \end{mathpar}
  \begin{center}
    (C) - Type Checking
  \end{center}
  \caption{Stream Operations}
  \label{fig:streams}
\end{figure*}

==> fig-syntax.tex <==
\begin{figure}
    \[
    \begin{array}{@{}p{1.7cm}r@{~}c@{~}l@{}}
      % {\small Ground types}
      % & \nu & \in & \GROUND
      % \\
      {\small Types}
      & \tau & \Coloneqq
      & \nu \mid \tyS{\tau} \mid
      \tyARR{\tau}{\tau} \mid \tyPROD{\tau}{\tau} \mid \tySUM{\tau}{\tau}
      \mid \tyW{p}{\tau}
      % \\
      % {\small Ground values}
      % & s & \in & \cup_{\nu \in \GROUND} \SCAL_\nu
      \\
      {\small Implicit terms}
      & t & \Coloneqq
      & x \mid \synFUN{x}{\tau}{t} \mid t~t
      \mid (t, t) \mid \synPROJ{i \in \{ 1, 2 \}}{t}
      \\ & & \mid &
      \synINJ{i \in \{ 1, 2 \}}{\tau}{t}
      \mid \synCASE{t}{x}{t}{x}{t}
      \\ & & \mid &
      s \mid \synREC{x}{\tau}{t} \mid \synBY{t}{p}
      \\
      {\small Coercions}
      & \alpha & \Coloneqq
      &
      \coeID \mid \alpha;\alpha
      \\ & & \mid &
      \coeS{\alpha}
      \mid \coeARR{\alpha}{\alpha}
      \mid \coePROD{\alpha}{\alpha}
      \mid \coeSUM{\alpha}{\alpha}
      \mid \coeW{p}{\alpha}
      \\ & & \mid
      &
      \coeWRAP \mid \coeUNWRAP
      \mid \coeCONCAT{p}{p} \mid \coeDECAT{p}{p}
      \\ & & \mid &
      \coeDISTP \mid \coeFACTP
      % \mid \coeDISTS \mid \coeFACTS
      \mid \coeINFL \mid \coeDEL{p}{p}
      \\
      {\small Ctx.~coercions}
      & \beta & \defeq
      & \mi{Var} \tofin \mi{Coe}
      \\
      {\small Explicit terms}
      & e & \Coloneqq
      &
      \renewcommand{\kw}[1]{\mt{#1}}
      \grayout{
        x \mid \synFUN{x}{\tau}{e} \mid e~e
        \mid (e, e) \mid \synPROJ{i \in \{ 1, 2 \}}{e}
      }
      \\ & & \grayout{\mid} &
      \renewcommand{\kw}[1]{\mt{#1}}
      \grayout{
        \synINJ{i \in \{ 1, 2 \}}{\tau}{e}
        \mid \synCASE{e}{x}{e}{x}{e}
      }
      \\ & & \grayout{\mid} &
      \renewcommand{\kw}[1]{\mt{#1}}
      \grayout{
        s \mid \synREC{x}{\tau}{e} \mid \synBY{e}{p}
      }
      \mid \synCOER{e}{\alpha} \mid \synCOEL{\beta}{e}
    \end{array}
  \]
  \caption{Syntax of Types, Terms, and Coercions}
  \label{fig:syntax}
\end{figure}


==> sec-implementation.tex <==
\section{Implementation}
\label{sec:implementation}

We have implemented the type-checking algorithm presented in this paper,
specialized to the class of time warps which can be presented as running sums of
ultimately periodic
sequences~\cite{CohenDurantonEisenbeisPagettiPlateau-POPL-2006,Plateau-2010}.
%
\iftoggle{fullversion}{\Refapp{effective-time-warps} contains additionals
  details and a link to the prototype.}{The appendix~\cite{APPENDIX} contains
  additionals details and a link to the prototype.}
%
It is able to type-check the following definition.
%
\[
  \small
  \begin{array}{r@{~}l}
    \kw{rec} ~
    \mt{nat} : \tyW{\pw{1\,0}}{\tyS{\tyI}}
    &
    =
    \synBY
    {
      (
      0 :: \mt{pos}
      )
    }{\pw{1\,0}}
    \\
    \kw{and} ~
    \mt{pos} : \tyW{\pw{0\,1}}{\tyS{\tyI}}
    &
    =
    \synBY
    {
      (
      \mt{map}~
      (\synFUN{\mt{x}}{\tyI}{\mt{x} + 1})~
      \mt{nat}
      )
    }{\pw{0\,1}}
  \end{array}
\]
%
The types~$\tyW{\pw{1\,0}}{\tyS{\tyI}}$ and~$\tyW{\pw{0\,1}}{\tyS{\tyI}}$
describe integer streams growing by one element at even and odd steps,
respectively.
%
They thus capture the growth patterns discussed in~\Refsec{introduction}.

